LSTM-Based Proactive Congestion Management for Internet of Vehicle Networks

Vehicle-to-everything (V2X) networks support a variety of safety, entertainment, and commercial applications. This is realized by applying the principles of the Internet of Vehicles (IoV) to facilitate connectivity among vehicles and between vehicles and roadside units (RSUs). Network congestion management is essential for IoVs and it represents a significant concern due to its impact on improving the efficiency of transportation systems and providing reliable communication among vehicles for the timely delivery of safety-critical packets. This paper introduces a framework for proactive congestion management for IoV networks. We generate congestion scenarios and a data set to predict the congestion using LSTM. We present the framework and the packet congestion dataset. Simulation results using SUMO with NS3 demonstrate the effectiveness of the framework for forecasting IoV network congestion and clustering/prioritizing packets employing recurrent neural networks.

==> CFP.tex <==
\textcolor{blue}{As one of the typical networking paradigms for Internet of Things, the Internet of Vehicles (IoV) enables seamless information dissemination and task processing among vehicles equipped with onboard sensing, communication, computing, and storage capabilities. With the development of advanced artificial intelligence (AI) techniques, it is envisioned to realize the ubiquitous intelligence for IoV. Different network entities including connected vehicles, wireless base stations, edge/cloud servers, aerial/space-assisted devices (e.g., drones, satellites), are expected to efficiently interact to perceive, reason, and make intelligent decisions based on context awareness for improving the networking and computing effectiveness. Highly responsive task computing, adaptive networking, and efficient resource control are imperative for the implementation of intelligent, safe, and ubiquitous IoV to satisfy increasingly differentiated vehicular application requirements
To realize the ubiquitous intelligence for IoV, further research endeavors are needed especially when high network complexity and vehicle mobility are present. On one hand, it is of paramount importance to explore how efficient AI frameworks are developed. For instance, hierarchical learning architectures can be investigated to fit in different IoV scenarios for improving the overall networking, computing, and control performance. On the other hand, technical challenges need to be overcome to deal with highly dynamic and complex vehicular network environments. Therefore, a practical implementation of AI modules can be achieved through balancing learning performance and complexity.
The objective of organizing this Special Issue (SI) is to attract and disseminate novel research ideas, concepts, approaches, and findings from both academia and industry to tackle challenges in developing effective and practical solutions for ubiquitous intelligence for IoV. Potential topics include but are not limited to:
Architectures, frameworks, and concepts for AI-enabled IoV
Intelligent networking and computing for autonomous driving
AI-enabled end-edge-cloud interplay for IoV
Intelligent communication, computing, and control for IoV
Edge intelligence for IoV
Vehicle-to-vehicle-assisted intelligent communication and computing
Intelligent space/air-assisted IoV
Distributed learning for IoV
Intelligent edge content caching for IoV
Intelligent multi-dimensional resource control for IoV
Intelligent security and privacy preservation for IoV
AI-based data analytics for IoV
Digital-twin-assisted intelligent IoV
Short-range wireless communication for IoV
Autonomous authentication and handover authentication in IoV
}
